Real-Time Reinforcement Learning for Vision-Based Robotics Utilizing Local and Remote Computers

Real-time learning is crucial for robotic agents adapting to ever-changing, non-stationary environments. A common setup for a robotic agent is to have two different computers simultaneously: a resource-limited local computer tethered to the robot and a powerful remote computer connected wirelessly. Given such a setup, it is unclear to what extent the performance of a learning system can be affected by resource limitations and how to efficiently use the wirelessly connected powerful computer to compensate for any performance loss. In this paper, we implement a real-time learning system called the Remote-Local Distributed (ReLoD) system to distribute computations of two deep reinforcement learning (RL) algorithms, Soft Actor-Critic (SAC) and Proximal Policy Optimization (PPO), between a local and a remote computer. The performance of the system is evaluated on two vision-based control tasks developed using a robotic arm and a mobile robot. Our results show that SAC's performance degrades heavily on a resource-limited local computer. Strikingly, when all computations of the learning system are deployed on a remote workstation, SAC fails to compensate for the performance loss, indicating that, without careful consideration, using a powerful remote computer may not result in performance improvement. However, a carefully chosen distribution of computations of SAC consistently and substantially improves its performance on both tasks. On the other hand, the performance of PPO remains largely unaffected by the distribution of computations. In addition, when all computations happen solely on a powerful tethered computer, the performance of our system remains on par with an existing system that is well-tuned for using a single machine. ReLoD is the only publicly available system for real-time RL that applies to multiple robots for vision-based tasks.

==> root-copy.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{RESULTS}
\begin{figure}
\centering
    \begin{subfigure}{.95\columnwidth}
        \includegraphics[width=\columnwidth]{create_reacher_all_runs_sac.png}
        \caption{Create-Reacher using SAC}
        \label{fig:create_reacher_sac}
    \end{subfigure}\hfill%
    \begin{subfigure}{.95\columnwidth}
        \includegraphics[width=\columnwidth]{ur5_reacher_all_runs_sac.png}
        \caption{UR5-VisualReacher using SAC}
        \label{fig:ur_reacher_sac}
    \end{subfigure}
\caption{Comparison of learning performance across different modes of the remote-onboard system using Soft Actor Critic. The onboard-only mode was unable to learn a policy using SAC. The solid lines for each mode are averaged over five independent runs. }
\label{fig:sac-all-modes}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{ur5_reacher_all_runs_ppo.pdf}
    \caption{UR5-VisualReacher using PPO. The solid lines for each mode are averaged over five independent runs.}
    \label{fig:ur_ppo}
\end{figure}

We show the learning curves of the three configurations of the SAC-agent in Fig. \ref{fig:sac-all-modes}. Note that the real experience time in our plots does not include additional components required to run an experiment, including resetting the environment and recharging the robot. Unfortunately, we were unable to run the local-only configuration for SAC-agent on Create-Reacher regardless of the choice of buffer size since Jetson Nano was unable to perform learning updates within a reasonable time frame. Each wide learning curve was the average of 5 independent runs of the same hyper-parameter configuration. The remote-local configuration outperformed the other two consistently and by a large margin on both tasks. In addition, the remote-only mode exhibited a much higher variance in overall learning performance. Surprisingly, the performance of the local-only configuration on the UR5-VisualReacher is very close to the remote-only though it uses much less resources.

The learning curves of the PPO-agent on UR5-VisualReacher is shown in Fig. \ref{fig:ur_ppo}. Each solid learning curve was the average of 5 independent runs of the same hyper-parameter configuration. The performance of the remote-local configuration was on par with local-only configuration here, while remote-only configuration was slightly worse than both.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{yufeng_ours_comparison.pdf}
    \caption{Comparing onboard-only mode of our system with an off-the-shelf implementation of \protect\citeA{yuan2021asynchronous} on a powerful workstation.  The solid lines for each mode are averaged over five independent runs. Both methods use SAC to learn a control policy. }
    \label{fig:yufeng_ours}
\end{figure}

We also compared our implementation in local-only mode with an off-the-shelf implementation of \citeA{yuan2021asynchronous}'s system in Fig. \ref{fig:yufeng_ours} using a powerful workstation. Both methods achieved similar overall learning performance. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Conclusions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{DISCUSSION \& CONCLUSIONS}
In this paper, we used our proposed remote-local system to compare the performance of three different distributions of computations of a learning system between a resource-limited local computer and a powerful remote computer. In total, we conducted 45 independent runs in our experiments, which took nearly 160 hours of usage on robots. We achieved effective learning without tuning the hyper-parameters, using only default hyper-parameters proposed by the original authors of PPO and SAC, which indicates the reliability of the algorithms, our learning system, and our task setup. The subtleties and interesting properties of real-time learning revealed by our experiments are summarized in this section.

\textit{Effects of latency in communicating actions and observation.} We believe that the relatively poor performance of remote-only mode in all tasks is primarily due to the variable latency in communicating actions and receiving observations over WiFi. \citeA{mahmood2018setting} showed that system delays occurring in different computational stages could be detrimental to learning. The variable latency of WiFi in our remote-only setup negatively impacted our learning system.

\textit{Comparison of SAC and PPO on UR5-VisualReacher.} In all of the three configurations, PPO takes much longer than SAC to learn a good policy and SAC achieves twice the return attained by PPO (see Fig. \ref{fig:ur_reacher_sac} and Fig. \ref{fig:ur_ppo} ). While SAC is more sample efficient since it can effectively leverage frequent off-policy gradient updates, it requires considerably more computational resources than PPO. Our results indicate that there exists a trade-off between the availability of computational resources and overall learning performance.  

\textit{Failure of SAC on Jetson Nano.} Unfortunately, we were unable to learn a good policy within a reasonable time frame on Create-Reacher with a Jetson Nano. The main problem is that each SAC update takes enormous time on both platforms (e.g., $\sim 87s$ on the Jetson Nano). Given a fixed learning period, the total number of learning updates performed by an agent is inversely correlated with the time required to make one SAC update. Considering that both tasks require tens of thousands of updates to achieve good performance, we determined it is impossible to finish the training within a reasonable time frame. Thus, we decided that the Jetson Nano does not have enough resources to take advantage of SAC. While SAC is more sample efficient than PPO, its computational requirements may prohibit us from successfully deploying it to  resource-limited local computers in local-only configuration. % However, as mentioned earlier, we could still deploy PPO and potentially achieve good learning performance, albeit at a much slower rate. 

%Our results show that the proposed \textit{remote-onboard} system successfully supported SAC and PPO on resource-limited computers such as Jetson Nano and Lenovo Ideapad Y700 Laptop in solving two real-time tasks, Create-Reacher and UR5-VisualReacher. 
Our results indicate that the remote-only configuration significantly suffers from variable delays in collecting observations and sending actions. 
On the other hand, the remote-local configuration seems to sidestep the latency issues, thus avoiding the pitfalls of remote-only learning. 
Our results also demonstrate that the performance of state-of-the-art RL algorithms can be compromised in the local-only configuration due to resource limitation.
In addition, our results verify our second hypothesis that when our system is configured to the local-only mode and deployed to a powerful workstation, its performance is on par with off-the-shelf systems that require lots of resources to enable real-time learning. Thus, our experiments support the claim that the remote-onboard system can help resource-limited computers leverage resource-demanding deep RL algorithms in an effective manner. 


\addtolength{\textheight}{-5cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section*{APPENDIX}

%Appendixes should appear before the acknowledgment.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{apacite}

\bibliography{refs}

\end{document}

